Stanley decompositions of rings of invariants and certain highest weight Harish-Chandra modules

The first half of this paper is largely expository, wherein we present a systematic combinatorial approach to the theory of polynomial (semi)invariants and multilinear invariants of several vectors and covectors, for the classical groups. This culminates in a graphical description of graded linear bases. By applying well-known results of lattice path combinatorics to Weyl's fundamental theorems of classical invariant theory, we write down Stanley decompositions and Hilbert-Poincare series in terms of families of non-intersecting lattice paths, enumerated with respect to certain corners. In the second half of the paper, we revisit the (semi)invariants in the first half as a special case of a much broader phenomenon. On one hand, polynomial invariants of a group $H$ can be generalized to modules of covariants, i.e., $H$-equivariant polynomial functions between $H$-modules. On the other hand, from the perspective of Roger Howe's theory of dual pairs, these modules of covariants can be viewed as infinite-dimensional simple $(\mathfrak{g}, K)$-modules. This suggests an expanded program in which our goal is to apply combinatorial techniques involving lattice paths in order to write down Hilbert series for arbitrary unitarizable highest-weight $(\mathfrak{g},K)$-modules. As a preview of future work in this program, we present examples showing how modules of covariants -- even those which are not Cohen-Macaulay, and therefore which we would not expect to be combinatorially nice -- can be decomposed in terms of lattice paths. We also extend these methods beyond the classical groups.

==> Assorted_notes.tex <==


Notes to self, about choice of positive roots:

For $\g = \sl_{p+q}$, we choose simple roots
\[
\alpha_i = 
\begin{cases}
\ep_{p-i+1} - \ep_{p-i},& 1 \leq i \leq p-1,\\
\ep_1 - \ep_{p+1} = \gamma_1,& i = p,\\
\ep_i - \ep_{i+1},& p+1 \leq i \leq p+q-1.
\end{cases}
\]
In this way, the poset $\Phi(\p^+)$ has minimal element $\al_p = \gamma_1$ in the upper-left, i.e., in the $(1,1)$ position.  If we write something like
\[
[a_1, \ldots, a_p; b_1, \ldots, b_q] \coloneqq (a_p, \ldots, a_1; b_1, \ldots, b_q),
\]
then we have
\[
\gamma_i = [0,\ldots,0,\underbrace{1,0,\ldots,0}_{i};\underbrace{0,\ldots,0,-1}_{i},0,\ldots,0] = (\underbrace{0,\ldots,0,1}_{i},0,\ldots,0;\underbrace{0,\ldots,0,-1}_{i},0,\ldots,0).
\]
Likewise, we have
\begin{alignat*}{4}
\omega_i &= [0^{p-i}, 1^p; 0^q] &&= (1^p, 0^{p-i}; 0^q), &&\quad 1 \leq i \leq p,\\
\omega_i &= [1^p; 1^{i-p},0^{p+q-i}] &&= (1^p; 1^{i-p},0^{p+q-i}), && \quad p+1 \leq i \leq p+q.
\end{alignat*}
% Now let's try to write down weights for $\k = \gl_p \oplus \gl_q$.  We have
% \[
% (-\omega_i, \omega_i) = (\underbrace{-1,\ldots,-1}_{i},0,\ldots,0;\underbrace{1,\ldots,1}_{i},0,\ldots,0) = -\sum_{j=1}^i \gamma_i.
% \]
% Therefore, in the language of \cite{GW}, the highest weight vector $\prod_i \Delta_i^{m_i} \in \C[\p^+]$ has weight 
% \[
%     \left(-\sum_i m_i \omega_i, \sum_i m_i \omega_i\right) = -\sum_i n_i \gamma_i,
% \]
% where $n_i = \sum_{j=i}^r m_j$, or equivalently, $m_i = n_i - n_{i+1}$.

% The $\k$-module generated by $\prod_i \Delta_i^{m_i}$ can be regarded as the span of bitableaux whose column lengths are $n_1, \ldots, n_r$; equivalently, the row lengths can be written out as $r^{m_r}, \ldots, 1^{m_1}$.  The left side has entries up to $p$, the right side up to $q$.  The highest weight vector corresponds to the bitableau where the $i$th column from the middle is filled with $i$'s all the way down. In other words, each row looks like $1,2,3,\ldots$.  Hence if we read this bitableau as the product of minors (with row indices on the left and column indices on the right), then we indeed recover $\prod_i \Delta_i^{m_i}$.

\subsection{Thoughts on covariants}\

Notation?  Define the facet set $\scrF_{k,m}$ containing all families of $k$ maximal non-intersecting paths in $\P_{\O}$, exactly $m$ of which have their endpoints on the diagonal ``painted.''  A painted endpoint does not count as a corner.  Let ${\rm end}(\f) \mathcal{C}^n_m$ denote the set of $m$ painted endpoints. For $I = (i_1, \ldots, i_m) \in \mathcal{C}^n_m$, define the function $\phi_I(v_1, \ldots, v_n) \coloneqq v_{i_1} \wedge \cdots \wedge v_{i_m}$.

\bigskip

\begin{theorem}
Let $H = \O_k$, and let $0 \leq m \leq k$.  Then we have the Stanley decomposition
\[
{\rm Cov}_H(V^n, \: \scalebox{.85}{$\bigwedge$}^{\!m} V) = \bigoplus_{\mathclap{\f \in \scrF_{k,m}}} f_{\cor(\f)} \: \C[f_{ij} \mid (i,j) \in \f] \cdot \phi_{{\rm end}(\f)} ,
\]
and the Hilbert series
\[
\frac{t^m\sum_{\f \in \scrF_{k,m}} (t^2)^{\#\cor(\f)}}{(1-t^2)^{k(2n-k+1)/2}}.
\]
\end{theorem}

We also have a basis of graphs in which $m$ vertices are painted.  Note that in $\P_{\O}$, we have $\scrF_k = \scrF_{k,0}$, and so we have $\#\scrF_{k,m} = \binom{k}{m}(\#\scrF_k)$.  This relates the Bernstein degrees for all $m=0, \ldots, k$.

\bigskip

\textbf{JUST NOTES \& MUSINGS AFTER THIS}


Example from Friday: 

\begin{itemize}
\setlength{\itemsep}{.5cm}
    \item $\g = \sp_{2n}$
    
    \item $\la = -\frac{k}{2} \omega_n + \omega^*_m = \big(\underbrace{-\tfrac{k}{2}, \ldots, -\tfrac{k}{2}}_{n-m}, \underbrace{-\tfrac{k}{2}-1, \ldots, -\tfrac{k}{2}-1}_{m}\big)$.

    \item This corresponds to $H = \O_k$ and $\sigma = (1^m)$.

    \item \textbf{CONJECTURE:} For $\sigma = (1^m)$, the Hilbert series of $\operatorname{Cov}_{H}(V^n, U_\sigma)$ is
    \[
    \frac{\binom{n}{m}}{\binom{m+n-k}{m}}\frac{\sum_\nu \dim \F{\nu}{n-k+1} t^{|\nu|}}{(1-t^2)^{k(2n-k+1)/2}} =
    \frac{t^m\sum_{\f \in \scrF_{k,m}} t^{2\cdot \#\cor(\f)}}{(1-t^2)^{k(2n-k+1)/2}},
    \]
    with the notation as follows:

    \begin{itemize}
        \item The sum on the left ranges over all $\nu \in \Par((n-k+1) \times k)$ with exactly $m$ odd columns.  (We already know that the left-hand side is true.)
        \item The facet set $\scrF_{k,m}$ contains all families of $k$ maximal non-intersecting paths in $\P_{\O}$, exactly $m$ of which have their endpoints on the diagonal ``painted.''
        \item A painted endpoint does not count as a corner.
    \end{itemize}
    
    \item It follows from the conjecture that the Bernstein degree equals $\binom{k}{m}(\#\scrF_k)$, for all $m = 0, \ldots, k$.  In other words, this is $\binom{k}{m}$ times the Bernstein degree of the $\O_k$-invariant ring.  Proof: each facet in $\scrF_k$ corresponds to $\binom{k}{m}$ facets in $\scrF_{k,m}$, one for each way to paint $m$ of the $k$ endpoints.

    \item Understanding the left-hand side:

    \begin{itemize}
        \item The RSK correspondence maps each tableau in $\bigcup_\nu \SSYT(\nu, \: n-k+1)$ to an upper-triangular matrix with trace $m$.  The multisupport decomposes into as many strict chains in $\P_{\O}(n-k+1)$ as there are columns in $\nu$.  By peeling off the multisupport into strict chains from SE to NW, we reconstruct the $k$ paths in a facet, as follows: any non-diagonal element is a corner, and any diagonal element is the painted endpoint in that column (specifically, 1 above).  We reconstruct the paths from bottom to top, by lining up upper-right corner of the RSK matrix immediately below $s_i$ (just as we did for the invariants and semi-invariants).

        \item Crucially, though, RSK cannot create all facets in $\scrF_{k,m}$, unless $m=0$ or $m=k$.  This explains the ``mystery ratio'' $\frac{\binom{n}{m}}{\binom{m+n-k}{m}}$, which scales up to make up for the missing facets.  The ``miracle'' is that this scaling preserves the proportions of facets containing each given number of corners; I still need to understand why this ratio of binomial coefficients is the right one.

        \item For the facets with 0 corners this is obvious, but beyond that, the justification for the mystery ratio is ... well, mysterious.

        \item Specific example from Friday: $n=4$, $k=2$, $m=1$.  There are 10 families of $k=2$ paths, which we multiply by $\binom{k}{m} = \binom{2}{1} = 2$ to obtain all 20 facets in $\scrF_{2,1}$.  When we do this, we observe that 4 facets have 0 corners, 12 facets have 1 corner, and 4 facets have 2 corners.  Counting each corner as degree-2, and multiplying through by $t_m = t$, we obtain $t+12t^3 + 4t^4$, which equals $\binom{4}{1}/\binom{3}{1} = 4/3$ times $\sum_\nu \dim\F{\nu}{n-k+1} t^{|\nu|}$.

        \item When we apply RSK to each tableau with the required shape, we obtain 3 facets with 0 corners, 9 facets with 1 corner, and 3 facets with 2 corners.  Clearly these are 3/4 of the final counts.

        \item Observation in this small example: the only facets that do not appear via RSK are those in which the painted endpoint lies 1 above the non-painted endpoint.  This is because when we unpeel these facets, the top path is no longer strictly above the bottom path in the RSK matrix, so the matrix we recover is the one where the painted endpoint was on bottom.

        \item In the mystery ratio, the numerator $\binom{n}{m}$ counts the number of ways to choose $m$ locations for the painted endpoints in $\P_{\O}$.  The denominator $\binom{m+n-k}{m}$ counts the number of ways to fill in the diagonal of the RSK matrix so that its trace is $m$.  In this example, there are 4 locations for endpoints, but only 3 diagonal spots in the RSK matrix.  Somehow, this means that the tableaux yield only 3/4 of the facets.  (This kind of makes sense, if you don't think about it too hard.)

        \item Another perspective on the denominator $\binom{m+n-k}{m}$: this is the number of ways to choose $m$ locations among all unpainted diagonal elements.  It's also the number of ways to choose non-endpoints among the unpainted diagonal elements.  This doesn't seem helpful, though.

        \item The mystery ratio simplifies to
        \[
        \frac{(n)_{k-m}}{(n-m)_{k-m}},
        \]
        where $(a)_b = a(a-1)\cdots(a-b+1)$ is the falling factorial.  This is the number of ways to choose the unpainted endpoints in order, divided by the number of ways to associate a non-painted diagonal element to each painted endpoint in order.  I can't think of a natural way to see this in the paths; the unsimplified form seems more promising.

        \item \textbf{Things that don't work:} I hoped that there was a nice way to individually scale up the facets we do obtain from tableaux, and then show that this averages out to our mystery ratio.  But in fact, given a number $c$ of corners, the tableaux do not always yield even one facet with $c$ corners which contains the correct paths.  So this is \textit{doubly} miraculous --- the mystery ratio knows exactly how to compensate for painted endpoints being switched for corners \emph{and} non-corners.
    \end{itemize}

    \item New example: $n=5$, $k=4$, $m=2$.  This time, the unscaled numerator is $3t^2 + 3t^4 + 3t^6$. The mystery ratio is $10/3$, so we end up with $t^2(10+10t^2+10t^4)$, which matches the 30 facets in $\scrF_{4,2} \subset 2^{\P_{\O}(5)}$.

    \item Once we prove the conjecture, we will have a very nice basis of graphs for $\operatorname{Cov}_H(V^n, \: U_{(1)^m})$: namely, the $\O_k$-invariant graphs where exactly $m$ of the vertices are painted.  This truly does ``interpolate'' the invariants and semi-invariants.  
    
    \item The painted vertices $i_1, \ldots i_m$ must mean something like $v_{i_1} \wedge \cdots \wedge v_{i_m}$.  Is it true that a basis for the covariants above is given by products of an invariant with a wedge product?

    \item Is the sum over all $m=0, \ldots, k$ anything interesting?  This has a basis of $\O_k$-invariant graphs in which an arbitrary number of vertices are painted.

    \end{itemize}

\subsection{Enright--Shelton reduction}







\newpage

\begin{center}\textbf{OLD NOTES:}\end{center}

\begin{itemize}

\item Observations on our previous results

\begin{itemize}
    
\item On one hand, we can write down a basis of either standard monomials or ordinary monomials, via RSK on SSYT's of the appropriate shape (mention that the ordinary monomials can be viewed as graphs via the Burge correspondence?):

\begin{itemize}
    \item Type I: $\bigcup_\mu \SSYT(\mu,p) \times \SSYT(\mu,q)$, where $\mu \in \Par(k \times \infty)$.

    \item Type II: $\bigcup_\mu \SSYT(\mu,n)$, where $\mu \in \Par(2k \times\infty)$ with even columns.

    \item Type IIIa: $\bigcup_\mu \SSYT(\mu,n)$, where $\mu \in \Par(k \times \infty)$ with even rows.

    \item Type IIIb: $\bigcup_\mu \SSYT(\mu,n)$, where $\mu \in \Par(k\times\infty)$ with odd rows.
\end{itemize}

\item On the other hand, we can write down Hilbert series in which the numerator polynomial is just the norm generating function of the SSYT's whose shapes are the conjugates of those above:

\begin{itemize}
    \item Type I: $\bigcup_\nu \SSYT(\nu, p-k) \times \SSYT(\nu, q-k)$, where $\nu \in \Par(\min\{p-k,q-k\} \times k)$.
    \item Type II: $\bigcup_\nu \SSYT(\nu,n-2k-1)$, where $\nu \in \Par((n-2k-1) \times 2k)$ with even rows.
    \item Type IIIa: $\bigcup_\nu \SSYT(\nu, n-k+1)$, where $\nu \in \Par((n-k+1) \times k)$ with even columns.
    \item Type IIIb: $\bigcup_\nu \SSYT(\nu,n-k+1)$, where $\nu \in \Par((n-k+1) \times k)$ with odd columns.
\end{itemize}

\item Early observation: the combinatorics here reminds one of the Enright--Shelton reduction in our first paper.  In Enright reduction, in order to pass from an infinite-dimensional module to its associated finite-dimensional module, we reduce the rank and ``switch'' between Types $\ssC$ and $\ssD$.  From the current perspective, in order to pass from an explicit basis of the infinite-dimensional module (parametrized by SSYT's) to the Hilbert series of its associated finite-dimensional module, we reduce the rank by the same amount and ``switch'' between Types $\ssC$ and $\ssD$, this time by transposing the Young tableau shapes.

\end{itemize}


\item Type IIIb: The standard monomial basis given by \cite{Domokos} yields a Stanley basis, but not of the form suggested by our table.  In fact, it is possible to find a decomposition with fewer summands by choosing a different monomial basis.

\begin{itemize}
    \item Domokos essentially states that his basis is indexed by SSYT's with odd rows.  We can interpret these as ordinary monomials $z_{\mathbf a} \cdot \text{product of }x_{ij}$'s, as follows. 
 The first column yields the $\mathbf a = (a_1, \ldots, a_k)$, while the remainder of the tableau (via Burge's RSK) yields a monomial in the $x_{ij}$. 
 When depicted on the usual poset, the support of the $x_{ij}$ lies in at most $k$ chains with starting points given by $\mathbf a$.  (Check this!)

 \item Therefore, in reverse, a Stanley basis is given by all families of $k$ non-intersecting paths with arbitrary (but distinct) starting points $\mathbf a$.  (The endpoints on the diagonal are already arbitrary.)  For each such family, $F_i$ is the union of the paths, while $\eta_i$ is the union of the corners (i.e., SW turns and S final segments) along with $z_\mathbf a$.  Note that each $\mathbf a$ determines the size of $F_i$, which are therefore NOT uniform.

 \item To fix this, we will introduce a new basis. 
 The basis elements are still monomials of the form $z_\mathbf a \cdot (\text{width $\leq k$ monomial in the $x_{ij}$})$, but this time, the support of the $x_{ij}$-monomial must lie on $k$ chains starting at $1, \ldots k$ and ending on the diagonal at $\mathbf a$.  In other words, these are the same basis monomials as in Type IIIa, but with ``extra information'' determined by the endpoints.  \textbf{I don't know yet how to read these directly from SSYT's --- it seems much harder than just stripping off the first column.  But it's also not necessary for our results.}

 \item Now, the better Stanley decomposition is given as follows.  Given a tableau with odd columns, use standard RSK on its twin-pair to obtain a symmetric matrix with trace $k$.  Ignore everything below the diagonal, of course.  Just as in IIIa, peel off the non-diagonal entries of the RSK matrix to determine the corner set $\eta_i$ (note that none of these occur on the diagonal of the big poset now --- show why!).  The diagonal of the RSK matrix gives $\mathbf a$ (just look directly north of each entry as you peel). Together, this suffices to determine the paths making up $F_i$.

 \end{itemize}

\item Types IIIc and IIId should be similar to IIIa and IIIb; see notes from 1/30, and make this precise.


\item Similar treatment for $\SL_k$-invariants?

\begin{itemize}
    \item By \cite{Lakshmibai}, we have a standard monomial basis, which we can index by pairs of SSYT's of the same shape, where exactly one of them has an arbitrary number of full columns appended in front.  (Call this number $m$, but make it negative if the extra columns are on the second tableau.)

    \item We can construct a Stanley decomposition from the ground up, similar to the first approach in IIIb, but this becomes complicated when $k$ and $\min\{p,q\}$ are far apart (unless $k=1$, which is trivial).  
    
    \item For $k=2$, we already know the Hilbert series from Type II where $k=1$.  But we can also interpret the combinatorics as follows. Let $\mathcal P(p,q)$ be the set of pairs of non-intersecting paths defined as follows:
    
    \begin{itemize}
        \item In a $p \times q$ rectangle, choose an arbitrary starting point $A = (a,1)$ along the west edge.  This determines a second starting point $B = (1, 3-a)$, along the westward extension of the north edge.  The endpoints are fixed at $C = (p,q-1)$ and $D = (p,q)$.  Now consider all pairs of non-intersecting paths $A \rightarrow C$ and $B \rightarrow D$.

        \item ``Reflect'' the setup above, so that $A$ can range along the bottom edge, $B$ lies along the southward extension of the east edge, and $C = (2,1)$ and $D = (1,1)$. Then consider paths $C \rightarrow A$ and $D \rightarrow B$.
    \end{itemize}
    
    Define a \emph{corner} of a path to be one of the following:
    
    \begin{itemize}
        \item a turn from south to east;
        \item the point where the path between $B$ and $D$ first intersects the edge of the rectangle, unless $B = (1,1)$.
    \end{itemize}
    
    Then the Hilbert series of $\C[V^p \oplus (V^*)^q]^{\SL_2}$ equals the following:
    \[
    \frac{\displaystyle\sum_{P \in \mathcal{P}(p,q)} (t^2)^{\text{\#corners of $P$}}}{(1-t^2)^{2(p+q)-3}}
    \]

    (There should be a corner-preserving bijection between $\mathcal{P}(p,q)$ and the set of all Dyck paths of semilength $p+q-2$.  What is it??)
    
    \item For $k > 2$, a similar interpretation should be possible, with families of $k$ non-intersecting paths.  But the ``external'' part of the longest path probably lies along a $k$-dimensional lattice --- in particular, a subgraph of the crystal graph of $\bigwedge^k \C^b$, that is, $\mathcal{B}_{(1^k)}$. (Here $b$ is the max of the starting points.) So we need to figure out a shelling for a $k$-dimensional poset; what is a ``corner'' in this setting? 

    \item I think Bj\"orner's idea of a ``lexicographically shellable'' poset might help us here.  Instead of labeling vertices by weights and edges by the Kashiwara operators (simple roots) $1, \ldots, b-1$, label the vertices by the actual $k$-sequence $(i_1, \ldots, i_k)$, and label an edge with $j$ if it corresponds to subtracting 1 from $i_j$.  Then (I think) the crystal graph is ``lexigraphically shellable'' in Bj\"orner's language, and therefore shellable.  I'll look up whether he gives an explicit recipe for the shelling.
    
    \item In general the denominator will take the form
    \[
    (1-t^2)^c (1-t^k)^d.
    \]

    \item We also used resolutions to sum up Hilbert series over all $m \in \mathbb Z$.
\end{itemize}

\begin{center}\includegraphics[height=10cm]{SL2 Hilbert series.pdf}\end{center}

\item Hilbert series of Wallach representations (outside the dual-pair setting)

\begin{itemize}
\item In each case, $\Phi(\p^+)$ can be given the structure of a poset whose $k$th order complex is pure and shellable.  (In simply-laced types, the poset structure coincides with the usual partial order on the roots.)

\item Therefore, we can use the methods from above to write the Hilbert series in terms of facets and minimal faces (``corners'').  \question{Do we get explicit Stanley decompositions for $\C[\overline{\mathcal O}_k]$ too, or is this not as straightforward?}

\item We again observe the shadow of Enright reduction: the complement of the first facet in the shelling has the structure of $\Phi(\p'^+)$.  \question{Can more be said, about dimensions of $\k'$-types, etc.?}

\item What is going on in  Type B?  We can easily impose a partial order on $\Phi(\p^+)$ that yields the correct Hilbert series, but it is completely artificial.  

\end{itemize}
\end{itemize}

Perhaps some useful terminology (according to \cite{Herzog08}):

Each summand $\eta_i \C[F_i]$ is called a \emph{Stanley space of dimension $|F_i|$}.  Given a Stanley decomposition, the minimum $|F_i|$ is called the \emph{Stanley depth} of the decomposition.
Likewise, the \emph{Stanley depth} of the entire ring (or module) is the maximum Stanley depth among all Stanley decompositions.  Stanley conjectured that the Stanley depth is always greater than or equal to the depth (in the usual sense).  

Billera et al.~ \cite{Billera} call the monomials in each $F_i$ the ``polynomial generators,'' and the monomials $\eta_i$ the ``separators.''

\cite{Murdock} also looks interesting.
\newpage


\bigskip

\hrule 

